One-loop impact factors for heavy quarkonium production: $S$-wave case

With the aim to extend the study of inclusive heavy quarkonium production at forward rapidities with the resummation of high partonic center-of-momentum-energy logarithms beyond Leading Logarithmic Approximation (LLA), the explicit analytic results for one-loop corrections to the following impact factors had been obtained: $\gamma R \to Q\bar{Q}\left[^1S_0^{[8]} \right]$, $g R \to Q\bar{Q}\left[^1S_0^{[1]} \right]$, $gR\to Q\bar{Q}\left[ ^1S_0^{[8]} \right]$ and $gR\to Q\bar{Q}\left[ ^3S_1^{[8]}\right]$, with $R$ being the Reggeized gluon and $Q$ is the heavy quark. The computation is done in the framework of Lipatov's gauge-invariant EFT for Multi-Regge processes in QCD with the tilted-Wilson-line regularisation for rapidity divergences. As expected, only single-logarithmic rapidity divergence proportional to the one-loop Regge trajectory of a gluon remains in the final result for impact-factors. Numerical comparison with Regge limits ($s/(-t) \gg 1$) of one-loop QCD amplitudes, described in the paper, provides a strong cross-check of obtained results. The relations of obtained results with other regularisation schemes for rapidity divergences used in low-$x$ physics, such as BFKL scheme, High-Energy Factorisation (HEF) scheme and shockwave scheme, are given.

==> 3S18_MI-expression.tex <==
 as:
\begin{eqnarray}
    C[X] &=& \frac{\bar{\alpha}_s}{4\pi} \left\{ c_1[X] A\left(\frac{M^2}{4}\right) + c_2[X] B(M^2,0,0) \right.  \nonumber \\
    &+& c_3[X] B\left( -\frac{M^2}{4}-\frac{{\bf k}_T^2}{2},0,\frac{M^2}{4} \right) + c_4[X] B(-{\bf k}_T^2,0,0) + c_5[X] B\left(-{\bf k}_T^2,\frac{M^2}{4},\frac{M^2}{4}\right) \nonumber \\
    &+& c_6[X] C\left(0,-\frac{M^2}{4}-\frac{{\bf k}_T^2}{2},\frac{M^2}{4};\frac{M^2}{4},\frac{M^2}{4},0\right) \nonumber \\
    &+& c_7[X] C\left(-\frac{M^2}{4}-\frac{{\bf k}^2_T}{2},-{\bf k}_T^2,\frac{M^2}{4};0,\frac{M^2}{4},\frac{M^2}{4}\right)  \nonumber \\
    &+& c_8[X] C\left( -\frac{M^2}{4}-\frac{{\bf k}_T^2}{2},-{\bf k}_T^2,\frac{M^2}{4};\frac{M^2}{4},0,0 \right) \nonumber \\
    &+& \left. c_9[X] C_{[+]}\left( k,0 ; \frac{p}{2}, \frac{M^2}{4} \right) + c_{10}[X] C_{[+]}\left( q,0 ; \frac{p}{2}-k,\frac{M^2}{4} \right) \right\},
\end{eqnarray}

where $\bar{\alpha}_s=g_s^2 r_\Gamma (\mu_R^2)^{-\epsilon}/(4\pi)^{1-\epsilon}$. The notation for scalar one-loop integrals without linear denominators is consistent with the standard notation for Passarino-Veltman functions, used e.g. in \texttt{LoopTools}~\cite{Hahn:1998yk}. In particular, the triangle integral with denominators $[l^2-m_1^2] [(l+p_1)^2-m_2^2] [(l+p_1+p_2)^2-m_3^2]$ is written as $C(p_1^2,p_2^2,(p_1+p_2)^2;m_1^2,m_2^2,m_3^2)$.  Coefficients corresponding to the LO Lorentz structure (\ref{eq:LO-ampl_g+R->3S18}) read:
\begin{eqnarray}
    c_1[{}^3S_1^{[8]},\text{LO}]&=&\frac{1}{M^2 ( M^2 + {\bf k}_T^2)^4 [d-5] [d-3] [d-1] [ M^2 + 2 {\bf k}_T^2]} \nonumber \\
    &\times& \left\{ -(C_A [ M^2 + 2 {\bf k}_T^2] [ ({\bf k}_T^2)^4 ( 152 - 250 d + 127 d^2 - 22 d^3 \right. \nonumber \\ 
    &&+ d^4) + 2 M^8 ( 26 - 80 d + 54 d^2 - 13 d^3 + d^4) \nonumber \\
    &&+ M^2 ({\bf k}_T^2)^3 ( 868 - 1382 d + 699 d^2 - 128 d^3 + 7 d^4) + M^6 {\bf k}_T^2 ( 628 \nonumber \\ 
    &&- 1154 d + 653 d^2 - 136 d^3 + 9 d^4) + M^4 ({\bf k}_T^2)^2 ( 1212 - 2030 d \nonumber \\ 
    &&+ 1101 d^2 - 216 d^3 + 13 d^4)]) + 2 C_F [ M^2 + {\bf k}_T^2] [ 2 ({\bf k}_T^2)^4 ( 42 - 83 d \nonumber \\ 
    &&+ 53 d^2 - 13 d^3 + d^4) + M^8 ( 82 - 161 d + 107 d^2 \nonumber \\
    &&- 31 d^3 + 3 d^4) + M^2 ({\bf k}_T^2)^3 ( 554 - 1053 d + 635 d^2 - 147 d^3 \nonumber \\
    && + 11 d^4) + M^6 ({\bf \
k}_T^2) ( 470 - 927 d + 597 d^2 - 153 d^3 + 13 d^4) \nonumber \\ 
&& \left.+ M^4 ({\bf k}_T^2)^2 ( 898 - 1741 d + 1075 d^2 - 251 d^3 + 19 d^4)] \right\}, 
\end{eqnarray}
\begin{eqnarray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
c_2[{}^3S_1^{[8]},\text{LO}]&=& \frac{-n_F}{( -2 + d)^2 ( M^2 + {\bf k}_T^2)^2 [ -1 + d]}  \Bigl( ({\bf k}_T^2)^2 ( -2 + d)^3 + 2 M^2 {\bf k}_T^2 [ -10 \nonumber \\ 
&&+ 12 d - 6 d^2 + d^3] + M^4 [ -4 + 12 d \nonumber \\ 
&&- 6 d^2 + d^3]\Bigr), \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
c_3[{}^3S_1^{[8]},\text{LO}]&=& \frac{- M^2}{2 ( M^2 + {\bf k}_T^2)^4 [ -2 + d] [ M^2 + 2 {\bf k}_T^2]} \Bigl( 4 C_F [ M^2 + {\bf k}_T^2] [ 4 M^6 ( -2 + d) \nonumber \\  
&& + 19 M^4 {\bf k}_T^2(-2 + d) + ({\bf k}_T^2)^3 ( -18 + 5 d)  \nonumber \\ 
&&+ 4 M^2 ({\bf k}_T^2)^2 (-13 + 6 d)] + C_A [ M^2 + 2 {\bf k}_T^2] [ M^6 ( 32 - 14 d + d^2) \nonumber \\ 
&&+ ({\bf k}_T^2)^3 ( 80 - 30 d + 3 d^2) + M^4 {\bf k}_T^2 ( 120 - 58 d + 5 d^2) \nonumber \\ 
 &&+ M^2 ({\bf k}_T^2)^2 ( 152 - 74 d + 7 d^2)]\Bigr) 
 \end{eqnarray}

\begin{eqnarray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
 c_4[{}^3S_1^{[8]},\text{LO}]&=&\frac{1}{2 ( -2 + d)^2 ( M^2 + {\bf k}_T^2)^4 [ -1 + d]} \Biggl\{ 2 n_F \Bigl( M^2 + {\bf k}_T^2\Bigr)^2 \Bigl[ ({\bf k}_T^2)^2 ( -4 + d)^2 + M^4 ( -2   \nonumber \\ 
 &&+ d)^2 + 2 M^2 {\bf k}_T^2 [ 6 - 6 d + d^2]\Bigr] + C_A 
\Bigl[ 4 d^4 M^2 {\bf k}_T^2 ( M^2 + {\bf k}_T^2)^2 \nonumber \\ 
&&+ 8 {\bf k}_T^2 [ 9 M^6 + 27 M^4 {\bf k}_T^2 + 31 M^2 ({\bf k}_T^2)^2 + 5 ({\bf k}_T^2)^3] + 4 d [ M^8 - 33 M^6 {\bf k}_T^2 \nonumber \\ 
&&- 101 M^4 ({\bf k}_T^2)^2 - 103 M^2 ({\bf k}_T^2)^3 - 12 ({\bf k}_T^2)^4] - 4 d^2 [ M^8 - 22 M^6 {\bf k}_T^2 - 68 M^4 ({\bf k}_T^2)^2 \nonumber \\ 
&&- 58 M^2 ({\bf k}_T^2)^3 - 5 ({\bf k}_T^2)^4] + d^3 [ M^8 - 28 M^6 {\bf k}_T^2 - 78 M^4 ({\bf k}_T^2)^2 - 52 M^2 ({\bf k}_T^2)^3 \nonumber \\
&&- 3 ({\bf k}_T^2)^4]\Bigr] \Biggr\},
\end{eqnarray}

\begin{eqnarray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
 c_5[{}^3S_1^{[8]},\text{LO}]&=& \frac{M^2 (C_A-2C_F)}{( M^2 + {\bf k}_T^2)^3 [ -2 + d]} [ 2 M^2 {\bf k}_T^2 ( 18 - 12 d + d^2) + ({\bf k}_T^2)^2 ( 20 - 10 d \nonumber \\
  &&+ d^2) + M^4 ( 8 - 6 d + d^2)], \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
 c_6[{}^3S_1^{[8]},\text{LO}]&=& \frac{-M^2 (C_A-2C_F)}{4 ( -2 + d) ( M^2 + {\bf k}_T^2)} \Bigl( {\bf k}_T^2 ( -4 + d)^2 + M^2 [ 20 - 8 d + d^2]\Bigr), \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
 c_7[{}^3S_1^{[8]},\text{LO}]&=& \frac{-M^2 (C_A - 2 C_F) }{( M^2 + {\bf k}_T^2)^2 [ -2 + d]} [ 2 M^2 {\bf k}_T^2 ( 22 - 12 d + d^2) + ({\bf k}_T^2)^2 ( 20 \nonumber \\
 &&- 10 d + d^2) + M^4 ( 16 - 6 d + d^2)] \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
 c_8[{}^3S_1^{[8]},\text{LO}]&=& \frac{C_A M^2 [ M^2 - {\bf k}_T^2] }{2 ( M^2 + {\bf k}_T^2)^4 [ -2 + d]}  [ M^6 ( -2 + d) + d M^4 {\bf k}_T^2 ( -1 \nonumber \\ 
 &&+ d) + ({\bf k}_T^2)^3 ( 16 - 7 d + d^2) + M^2 ({\bf k}_T^2)^2 ( 10 - 9 d \nonumber \\
 &&+ 2 d^2)], \\
 c_9[{}^3S_1^{[8]},\text{LO}]&=&\textcolor{red}{-} C_A q_+ {\bf k}_T^2 , \\
 c_{10}[{}^3S_1^{[8]},\text{LO}]&=& \textcolor{red}{-}C_A q_+ ( M^2 + {\bf k}_T^2).
\end{eqnarray}

For the mass-derivative Lorentz structure (\ref{eq:Mass-der:gR-3S18}), only the coefficient in front of $A(M^2/4)$ is nonzero:
\begin{equation}
    c_1[{}^3S_1^{[8]},\partial_{m_Q}\text{LO}] = \frac{(d-2)(d-1)C_F}{M(d-3)}.
\end{equation}

For the Lorentz-structure (\ref{eq:gR-3S18:LS1}) the nonzero coefficients read:
\begin{eqnarray}
    c_1[{}^3S_1^{[8]},\text{LS-1}] &=& \frac{1}{( M^2 + {\bf k}_T^2)^4 [ -3 + d] [ -1 + d] [ M^2 + 2 {\bf k}_T^2]} \nonumber \\ &\times & \Biggl\{ -4 C_F [ M^2 + ({\bf k}_T^2)] [ 2 ({\bf k}_T^2)^3 ( -13 + 21 d - 9 d^2 \nonumber \\ 
    &&+ d^3) + M^6 ( -4 + 7 d - 4 d^2 + d^3) \nonumber \\ 
    &&+ 2 M^4 ({\bf \
k}_T^2) ( -13 + 23 d - 12 d^2 + 2 d^3) + M^2 ({\bf k}_T^2)^2 ( \nonumber \\ 
&&-52 + 89 d - 42 d^2 + 5 d^3)] + C_A [ M^2 + 2 ({\bf k}_T^2)] [ M^6 ( 20 \nonumber 
\\
&&- 14 d + d^2 + d^3) + ({\bf k}_T^2)^3 ( -52 + 66 d \nonumber \\ 
&&- 25 d^2 + 3 d^3) + M^4 ({\bf k}_T^2) ( -4 + 30 d - 23 d^2 \nonumber \\
&&+ 5 d^3) \
+ M^2 ({\bf k}_T^2)^2 ( -60 + 94 d - 49 d^2 + 7 d^3)]\Biggr\},
\end{eqnarray}

\begin{eqnarray}
     c_2[{}^3S_1^{[8]},\text{LS-1}] &=& \frac{4 M^2 n_F ( M^2 - {\bf k}_T^2)}{( -2 + d)^2 ( M^2 + {\bf k}_T^2)^2 [ -1 + d]} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     c_3[{}^3S_1^{[8]},\text{LS-1}] &=& \frac{M^2}{2 ( M^2 + ({\bf k}_T^2))^4 [ -2 + d] [ M^2 + 2 ({\bf k}_T^2)]} \nonumber \\ 
     && \Bigl( 4 C_F [ M^2 + ({\bf k}_T^2)] [ 4 M^6 ( -2 + d) + 19 M^4 ({\bf k}_T^2) ( -2 \nonumber \\ 
     &&+ d) + ({\bf k}_T^2)^3 ( -18 + 5 d) + 4 M^2 ({\bf k}_T^2)^2 ( \
-13 \nonumber \\
&&+ 6 d)] + C_A [ M^2 + 2 ({\bf k}_T^2)] [ M^6 ( 32 - 14 d + d^2) + ({\bf k}_T^2)^3 ( 80 \nonumber \\
&&- 30 d + 3 d^2) + M^4 ({\bf k}_T^2) ( \
120 - 58 d + 5 d^2) + M^2 ({\bf k}_T^2)^2 ( 152 \nonumber \\ 
&&- 74 d + 7 d^2)]\Bigr), \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
c_4[{}^3S_1^{[8]},\text{LS-1}] &=& \frac{1}{2 ( -2 + d)^2 ( M^2 + ({\bf k}_T^2))^4 [ -1 + d]} \\
&\times & \Bigl\{ -2 n_F \Bigl( M^2 + ({\bf k}_T^2)\Bigr)^2 \Bigl[ ({\bf k}_T^2)^2 ( -4 + d)^2 + M^4 ( \nonumber \\
&&-2 + d)^2 + 2 M^2 ({\bf k}_T^2) [ 6 - 6 d + d^2]\Bigr] - \
C_A \Bigl[ \nonumber \\
&&-(({\bf k}_T^2)^4 ( -4 + d)^2 [ -2 + d]) + M^8 ( \nonumber \\
&&-2 + d)^2 [ -2 + 3 d] + 4 M^2 ({\bf k}_T^2)^3 [ 54 - 87 d 
\nonumber \\
&&+ 48 d^2 - 11 d^3 + d^4] + 4 M^6 ({\bf k}_T^2) [ 10 - 17 d + 12 d^2 \nonumber \\
&&- 5 d^3 + d^4] + 2 M^4 ({\bf k}_T^2)^2 [ 84 - 154 d + 106 \
d^2 - 33 d^3 \nonumber \\
&&+ 4 d^4]\Bigr] \Bigr\},
\end{eqnarray}

\begin{eqnarray}
    c_5[{}^3S_1^{[8]},\text{LS-1}] &=& \frac{-M^2 [ C_A - 2 C_F]}{( M^2 + ({\bf k}_T^2))^3 [ -2 + d]}  [ 2 M^2 ({\bf k}_T^2) ( 18 - 12 d + d^2) + ({\bf k}_T^2)^2 ( 20 \nonumber \\
    &&- 10 d + d^2) + M^4 ( 8 - 6 d + d^2)], \\
    c_6[{}^3S_1^{[8]},\text{LS-1}] &=& \frac{M^2 ( C_A - 2 C_F)}{4 ( -2 + d) ( M^2 + ({\bf k}_T^2))} \Bigl( ({\bf k}_T^2) ( -4 + d)^2 + M^2 [ 20 - 8 d + d^2]\Bigr), \\
    c_7[{}^3S_1^{[8]},\text{LS-1}] &=& \frac{M^2 (C_A - 2 C_F)}{4 ( M^2 + ({\bf k}_T^2))^2 [ -2 + d]} [ 2 M^2 ({\bf k}_T^2) ( 22 - 12 d + d^2) + ({\bf k}_T^2)^2 ( 20 - 10 d \nonumber \\
    &&+ d^2) + M^4 ( 16 - 6 d + d^2)], \\
    c_8[{}^3S_1^{[8]},\text{LS-1}] &=& \frac{-C_A M^2 [ M^2 - ({\bf k}_T^2)]}{2 ( M^2 + ({\bf k}_T^2))^4 [ -2 + d]}  [ M^6 ( -2 + d) + d M^4 ({\bf k}_T^2) ( \nonumber \\
    &&-1 + d) + ({\bf k}_T^2)^3 ( 16 - 7 d + d^2) + M^2 ({\bf k}_T^2)^2 ( 10 \
\nonumber \\
&&- 9 d + 2 d^2)].
\end{eqnarray}

The nonzero coefficients for the second Lorentz structure (\ref{eq:gR-3S18:LS2}) are:
\begin{eqnarray}
    c_1[{}^3S_1^{[8]},\text{LS-2}] &=& \frac{( -2 + d )}{( M^2 + ({\bf k}_T^2))^3 [ -3 + d] [ -1 + d]} \Bigl( 4 C_F [ -1 + d] [ M^2 + ({\bf k}_T^2)] [ ({\bf k}_T^2) ( \nonumber \\
&&-5 + d) + 2 M^2 ( -3 + d)] - C_A [ ({\bf k}_T^2)^2 ( 16 \nonumber \\ 
&&- 15 d + 3 d^2) + M^4 ( 12 - 11 d + 3 d^2) + 2 M^2 ({\bf k}_T^2) ( 12 \nonumber \\
&&- 11 d + 3 d^2)]\Bigr), \\
c_2[{}^3S_1^{[8]},\text{LS-2}] &=& \frac{-2 M^2 n_F}{( -2 + d) ( -1 + d) ( M^2 + ({\bf k}_T^2))}, \\
c_3[{}^3S_1^{[8]},\text{LS-2}] &=& \frac{M^2}{2 ( M^2 + ({\bf k}_T^2))^3} \Bigl( C_A [ 2 d M^2 ({\bf k}_T^2) + M^4 ( -2 + d) + ({\bf k}_T^2)^2 ( 6 + d)] \nonumber \\
&&- 4 C_F [ M^2 + ({\bf k}_T^2)] [ M^2 ( -2 + d) + ({\bf k}_T^2) ( -3 \nonumber \\
&&+ 2 d)]\Bigr), \\
c_4[{}^3S_1^{[8]},\text{LS-2}] &=& \frac{1}{2 ( M^2 + ({\bf k}_T^2))^3 [ -2 + d] [ -1 + d]} \nonumber \\
&\times & \Bigl\{ 2 n_F \Bigl( M^2 + ({\bf k}_T^2)\Bigr)^2 \Bigl[ ({\bf k}_T^2) [ -4 + d] + M^2 [ -2 \nonumber \\
&&+ d]\Bigr] + C_A \Bigl[ M^2 ({\bf k}_T^2)^2 ( -2 + d)^2 [ 
-11 + 4 d] \nonumber \\
&&- ({\bf k}_T^2)^3 [ 8 - 6 d + d^2] + M^6 [ 4 - 8 d + 3 d^2] \nonumber \\
&&+ M^4 ({\bf k}_T^2) [ -16 + 22 d - 15 d^2 + 4 d^3]\Bigr] \Bigr\},
\end{eqnarray}

\begin{eqnarray}
  c_5[{}^3S_1^{[8]},\text{LS-2}] &=& \frac{M^2 (C_A - 2 C_F)}{( M^2 + ({\bf k}_T^2))^2} [ M^2 ( -4 + d) - ({\bf k}_T^2) ( 2 + d)], \\
  c_6[{}^3S_1^{[8]},\text{LS-2}] &=& -\frac{1}{4}M^2 ( C_A - 2 C_F) ( -4 + d) , \\
  c_7[{}^3S_1^{[8]},\text{LS-2}] &=& \frac{-M^2 ( C_A - 2 C_F) [ -d {\bf k}_T^2 + M^2 ( -2 + d)]}{ 4 ( M^2 + ({\bf k}_T^2)) } , \\
  c_8[{}^3S_1^{[8]},\text{LS-2}] &=&  \frac{C_A M^2 [ M^2 - {\bf k}_T^2] [ M^4 + d M^2 ({\bf k}_T^2) + ({\bf k}_T^2)^2 ( -3 + d)]}{2 ( M^2 + ({\bf k}_T^2))^3}.
\end{eqnarray}
